Augmenting Zero-Shot Dense Retrievers with Plug-in Mixture-of-Memories

In this paper we improve the zero-shot generalization ability of language models via Mixture-Of-Memory Augmentation (MoMA), a mechanism that retrieves augmentation documents from multiple information corpora ("external memories"), with the option to "plug in" new memory at inference time. We develop a joint learning mechanism that trains the augmentation component with latent labels derived from the end retrieval task, paired with hard negatives from the memory mixture. We instantiate the model in a zero-shot dense retrieval setting by augmenting a strong T5-based retriever with MoMA. Our model, MoMA, obtains strong zero-shot retrieval accuracy on the eighteen tasks included in the standard BEIR benchmark. It outperforms systems that seek generalization from increased model parameters and computation steps. Our analysis further illustrates the necessity of augmenting with mixture-of-memory for robust generalization, the benefits of augmentation learning, and how MoMA utilizes the plug-in memory at inference time without changing its parameters. We plan to open source our code.

==> Arxiv/abs.tex <==

\begin{abstract}



In this paper we explore the potential of augmenting language models with plug-in mixture-of-memories, using a new mechanism that retrieves augmentations (``external memories'') from multiple information sources, and the ability to plug-in a new resource at serving time to incorporate in-domain information. 
Towards this goal we develop a new learning method that jointly trains the augmentation component with the language model to learn the memory mixture, which derives pseudo labels from the end task supervision and pairs them with hard negatives from the mixed information sources.
We use this plug-in mixture-of-memories scheme to augment a zero-shot dense retriever and evaluate the result system, \model{}, on the standard zero-shot retrieval benchmark, BEIR.
Our experiments demonstrate the advantage of \model{} over recent state-of-the-arts dense retrievers in zero-shot generalization ability, the benefit of augmentations from multiple resources, and the advantage of plug-in memory. 
Our analysis further illustrate how the joint learning helps \model{} utilize the mixture-of-memories and the benefits of in-domain information at serving time. We plan to open source our code. 
\end{abstract}

==> Arxiv/eva.tex <==
\section{Evaluation Results}



\subsection{Zero-Shot Retrieval Accuracy}
\input{Tables/main_res.tex}
\cx{Table: our best model versus fair baselines}

\cx{show how our method performance better than previous methods}



\subsection{Performance with Different Memories}
\input{Tables/05_1_mixture_table.tex}
\input{Tables/05_2_distill_tabel.tex}

\cx{Table: results without different augmented corpus: no augmentation, MARCO only, no target mixture, no mixture learning and direct usage in testing}

\cx{The goal is to show the benefits of mixture and plug-in switch}

\cx{Lead to the mixture learning analysis in next subsection}

\subsection{Effect of Memory Mixture Learning}
\label{sec:exp_distill}

\input{Figures/fig_learning.tex}

\cx{Table: show different performance of the distillation technique, how we learn from that soft label with pseudo labels constructed from it, versus RAG's basic strategies}

\cx{to show what has been learned in the mixture: \begin{enumerate}
    \item Figure: the change of weights on the corpus (FiD attention scores) during training and in testing)
    \item Figure: the fraction of documents from different sources (MARCO rel, irrelevant, Wiki, MeSH) in different checkpoints (ANCE episodes) and in testing time
\end{enumerate}
}
    

\cx{the goal is to demonstrate the benefits of our learning strategy, that the soft labels make sense, and the grounding is able to learn it, also how the hot-switch works in testing time}


\subsection{Effectiveness of Plug-In Memory}

\subsection{Case Studies}

\cx{Table: show examples on three main things: how the retrieval augmentation in general helps better q representation, how grounding on mixture instead of MARCO only helps, and how the hot switch to adding target corpus helps}









==> Arxiv/intro.tex <==
\section{Introduction}



% \cx{Main Contribution:
% \begin{enumerate}
%     \item augment representation models by retrieving from a set of corpus, with hot switch to corpus that may better aligns with target domain to improve zero-shot performance (plug-in mixture of memories).
%     dense retriever with plug-in mix of memory  improves zero-shot performance
%     \item a learning mechanism that leverages final supervision to help learn the mixture of grounding corpus
%     \item strong zero-shot performance on BEIR in domain generalization with or without target corpus in the testing time, with insights on how the model learns to retrieve and utilize augmented information from mixture of memories
% \end{enumerate}
% }


% \cx{Figure 1 a general figure to show the idea of plug-in new memory to the mixture in testing time for zero-shot}


% \cx{Per paragraph outline: from the POV of retrieval Aug for LM to improve generalization ability
% \begin{enumerate}
%     \item P1: Augment LMs with retrieved information provide various benefits in more efficient generalization,
%     \item P2: most augmentation is on a given corpus and treated as the general memory bank, but many times there are multiple possible resources, e.g., wiki, KG, and web corpus. also different target zero-shot scenarios may have different needs of retrieved memory
%     \item P3: in this work we study to possibility to augment representation models by retrieving from a set of corpus, providing a mixture of memory support to improve generalization ability. This also make it easy to plug in different memory component into the mixture based on target tasks' needs.
%     \item P4: More specifically, we choose zero-shot dense retrieval (ZeroDR) as the application scenario, we use retrieval augmentation to improve the query representation (the traditional IR query expansion setting).  (Describe how we do this in the general setup. 
%     \item P5: discuss the learning method we use to learn the mixture from the final supervision,  and how we plug-in the new memory in testing with prompts
%     \item P6: overall evaluation results and ablation studies
%     \item P7: the key findings we have in analysis, share out main insights in the analysis part of the evaluation results section.
% \end{enumerate}
% The main tricky part here is how we shrink the general retrieval augmentations representation part to using ZeroDR as the application to verify our modeling scheme. The importance of ZeroDR in real world is the key to make this justification. Also we can argue it is more convincing as it shows improvements on retrieval itself? We shall prepare for another application for rebuttal as reviewers will ask for another application scenarios I guess. At the same time I think this story flow is better than starting from the retrieval application POV as our motivation is more general than retrieval application?
% }


Scaling up language models---making them bigger, pretraining with more computation, and on more data---is known to improve model generalization ability on downstream applications ~\citep{raffel2019t5, brown2020language, rae2021scaling, chowdhery2022palm, smith2022using}.
However, various empirical observations also converge on the exponential scaling law of language models, showing  a \textit{linear} improvement on downstream applications often requires \textit{exponentially} more parameters and computing cost~\citep{kaplan2020scaling, hoffmann2022training}. 
After models reached hundreds of billions parameters, improving via scaling is unlikely sustainable, even for places with ample computing budgets~\citep{zhang2022opt}, and also raises  concerns on its influences on our environment and society~\citep{strubell2020energy, bender2021dangers}.


How to obtain generalization power more efficiently from language models without solely relying on scale is a critical, if not necessary, research direction in AI.
One promising path is retrieval augmentation, which enhances language models with access to top documents retrieved from a given corpus as external information~\citep{guu2020realm, borgeaud2022improving}, an ``open-book'' setting where the language models can leverage the retrieved information as a lookup augmenting memory in their learning and prediction. 
The augmenting memory alleviates language models from the trouble of memorization using their parameters~\citep{roberts2020much}.
Recent research demonstrates that using a single lookup memory can significantly improve the efficiency of language models, achieving similar generalization power with orders of magnitudes fewer parameters and computing costs~\citep{khandelwal2019generalization, borgeaud2022improving, izacard2022few}.


% the general idea of this model
% in this paper we aim to improve retrieval augmented model using mix of memories
In this paper we continue the development on retrieval augmented language models with a new augmentation mechanism: plug-in mixture-of-memory augmentation (MoMA).
% As illustrated in Figure~\ref{fig:intro}, 
Instead of sticking to one single retrieval corpus throughout training and testing,
we explore the potential of retrieval from multiple corpora that covers a variety of information resources, in order to provide a more robust augmentation to language models and enhance their generalization power to diverse downstream scenarios.
In addition, we also enable the model to switch to a completely unseen retrieval corpus that is only provided at testing time, for example, as a user designated ``plug-in'' memory.
% that better fits deploying scenario.
This memory switching mechanism enables a new way to incorporate a user's preference and domain knowledge at deploy time for better generalization, without any modification of model parameters or training process.





% \begin{wrapfigure}{r}{6cm}
% \centering
% \includegraphics[width=\textwidth]{Figures/intro.pdf}
% \caption{An illustration of target query augmentation with plug-in mixture-of-memory.\label{fig:intro}}
% \end{wrapfigure}

% as the first step, we choose the zero-shot retrieval as the application for our exploration.
% why? 1) an important real world as the end goal 2) also dense retrieval is the component to provide retrieval augmentation for LM, in both pretraining and fine-tuning.
We apply MoMA on zero-shot dense retrieval (ZeroDR), an important end application of many real-world systems~\citep{thakur2021beir}, and also the retrieval component of many retrieval augmented language models~\citep{guu2020realm, izacard2022few}.
We follow the standard setting of ZeroDR with a training phrase on a source retrieval task (web search), and then testing upon unseen retrieval scenarios from various domains, such as medical search.
In our \model{} system,  during training, the mixture-of-memory is composed by the source task's web corpus, Wikipedia, and a medical knowledge graph.
When testing, the source corpus is swapped out for the target retrieval corpus, and the model's augmentation mechanism adapts to the new domain's information with no modification of the model parameters.


Learning how to retrieve useful information from multiple corpora is challenging.
% Transition from a single memory to a mixture requires learning to retrieve useful information from the mixtures, which is not trivial as
No training signals are available except on the source corpus.
We develop a new joint training strategy that learns the augmentation component directly from source task relevance labels in an iterative manner with the retrieval model.
In each iteration, the augmentation component is trained by pseudo-labels derived from the retrieval model's attention on augmented documents~\citep{dong2019unified} and hard negatives from the corpus pool~\citep{xiong2020approximate}. The pseudo label training signal also back-propagates to the representations of augmented documents themselves, which the retrieval model is retrained to leverage in the next iteration.
This iterative approach naturally pairs with the standard iterations in dense retrieval training thus can be conducted without additional cost in comparison to the naive augmentation models.


% \cx{experimental overall results}
Our experiments on eighteen retrieval tasks included in the BEIR benchmark, the standard ZeroDR test bed~\citep{thakur2021beir}, demonstrate the advantage of \model{}.
Over either non-augmented language models -- or models only augmented from the source corpus --
\model{} shows stronger and more robust zero-shot accuracy on many unseen target domains.
It significantly outperforms a recent state-of-the-art ZeroDR system which also builds upon T5$_\text{base}$ but introduces additional training data in both pretraining and fine-tuning.
Our ablations studies show the empirical effectiveness of \model{} comes from the additional information retrieved from multiple corpora, the in-domain information from the plugged in target corpus, and the learning mechanism that enable the model to find the right combination of augmented documents.

\cx{how our model learns to leverage the mixture, and how the switching to new target actually works.}
\cx{examples of how model leverages MoM/target at zero-shot testing time.}
\cx{I will wait for analysis results to write this paragraph, otherwise it is just making up stuff.}















% our method: MoMA








==> Arxiv/model.tex <==
\section{Method}

\begin{figure*}[h]
\centering
\includegraphics[width=0.9\textwidth]{Figures/approach.pdf}
\caption{
% An illustration of learning to MoMA jointly with end task. 
% The supervision signal from the end retrieval task first back-propagates to the augmented query $\mathbf{q}_{aug}$. 
% The $\mathbf{q}_{aug}$ distributes the signal to each concatenated vector $\mathbf{g}_{i}$ according to its aggregated attention score via the grounding weight $w_i$.
% To differentiate useful grounding documents from uninformative ones, we rank all grounding weights $w_{1:k}$.
% We then transform each $w_i$ to a polarized pseudo label $w'_i$ according to its ranking, where $w'_i=1$  indicates a relevant grounding document and vice versa.
% We then leverage the pseudo label $w'_i$ to train the grounder by aligning its predicted probability $f(q,g'_i)$ with $w'_i$.
}
\end{figure*}

% \cx{I think we can follow a standard way to describe our method.
% Start with general zero-shot DR task, the Mixture-of-Memory Augmentation, the prompt tokens marking the memory source, the training of the retriever jointly with the augmentation components, the inference and the plug-in switch with new memory in target zero-shot scenario when see fit.
% }


% \cx{start this section following the discussion in the last paragraph of related work, describe why we choose ZeroDR as our application to demonstrate the advantage of MoMA. 1) it being one of the most important real-word application 2) Because the retrieval augmentation is not necessary in the task design, showing improve zero-shot ability is more convincing?}


% \cx{from a quick glance section 3's fraction of text versus equation is not quite right, there is too much texts over equations.}

% \textbf{Preliminaries.} 
% Dense Retrieval, Task, Zero-shot. (Training maybe can wait to describe with our joint learning.)

\textbf{Preliminaries.} Dense Retrieval (DR) represents each query or document as a dense vector using query and document encoder.
In this work, we use one encoder-decoder based T5 model~\citep{raffel2019t5} as the dual encoder for query and document.
Since our T5 decoding objective is a single query vector, following Sentence-T5~\citep{ni2022sentence}, we take the first decoder output (token position 0) as the sentence embedding. 
The ranking relevance score $g$ between query $q$ and candidate document $d^c$ is computed as the similarity between their encoded vectors:
\begin{equation}
    g(q, d^c)=\text{sim}(\mathbf{q}, \mathbf{d}^c), 
    \mathbf{q}=\text{Dec}(\text{Enc}(q)),
    \mathbf{d}^c=\text{Dec}(\text{Enc}(d^c)).
\end{equation}




A DR scenario is considered zero-shot if there is no supervision available from the target domain.
% ZeroDR is a practical scenario when manual annotation requires heavy labor and expertise, such as in medical and financial domains.
A common ZeroDR setup treats the target corpus as the most accessible in-domain information and performs unsupervised domain adaption on it.
However, the above setting may not hold for certain privacy-sensitive or low-resource retrieval scenarios, where the target corpus is not readily available in training. 
It requires the ZeroDR model to accommodate unseen plug-in corpus in inference, which is challenging to existing zero-shot methods.

% The general set up, definition of notations in the multiple corpus, and the FiD framework.
\textbf{Mixture-of-Memory Augmentation.} 
To improve the generalization of query representation, we propose to augment each query using documents from a mixture of memories $\mathcal{M}=\{C_s,C_1,C_2,...,C_M\}$, where $C_s$ is the source corpus, $C_{1:M}$ are $M$ different memory corpora ranging from general encyclopedia to domain-relevant databases.
One straight-forward solution to retrieve from the mixture $\mathcal{M}$ is searching over each memory component $C_i$ separately and merging the results.
However, it would be difficult to balance between the relevant importance of augmentation documents from different memory components.
Thus we train the memory component to automatically balance different memories and retrieve the top $K$ documents $\{d_1,...,d_K\} \in \mathcal{M}$ as augementation set $A_K$ by performing a one-time inference over $\mathcal{M}$.

One naive approach to synthesize information from multiple augmenting documents is to append all their constituent tokens as an augmented query $\mathbf{q_{\text{aug}}}=\text{Dec}(\text{Enc}([q,d_1,...,d_K]))$.
Unfortunately, this approach is not scalable for two reasons: the attention between tokens from different documents will result in a quadratic complexity with respect to $K$; and secondly the number of tokens that can fit into an encoder is limited in most large language models, meaning that some augmenting documents will have to be truncated or discarded entirely.

To alleviate this challenge, we incorporate a Fusion-in-Decoder (FiD) mechanism which increases the model's capacity for attending over multiple documents while remaining computationally efficient~\citep{izacard2020distilling}. The FiD framework separately encodes each document in the encoder.
During decoding, it concatenates the encoder's representations from each document into a single sequence and perform cross-attention when generating output tokens.
The augmented query is denoted as  $\mathbf{q_{\text{aug}}}=\text{Dec}([\text{Enc}(d_1),...,\text{Enc}(d_K)]))$.
We also append query to the beginning of all augmentation documents with a special [SEP] token separating all documents.
The \model{} augmented query vector $\mathbf{q}_{\text{aug}}$ is formulated as:
\begin{align}
    \mathbf{q}_{\text{aug}}&=\text{Dec}([\text{Enc}(q), \text{Enc}(\text{[SEP]} d_1),...,\text{Enc}(\text{[SEP]} d_K)])).
\end{align}

The augmented query $\mathbf{q}_{\text{aug}}$ is used for retrieval on the target corpus to generate the final relevance prediction $g(q_{\text{aug}}, d^c)=\text{sim}(\mathbf{q}_{\text{aug}}, \mathbf{d}^c)$.

% \corby{At this point, it is still not clear from this paper that there are two retrievers: a grounded retriever and an "outer" retriever. Nor is there a mention of "pseudo-relevance feedback" which if mentioned, is something a lot of people would immediately understand. This point must be made clearer}

\textbf{Learning to MoMA jointly with End Task.}
The key challenge in MoMA training is the lack of direct supervision for deriving augmentation set $A_K$ from $\mathcal{M}$.
One intuitive design would be guiding the augmentation component with relevance labels from the end task.
However, it may be sub-optimal since
1) relevance may not be the optimal searching goal of augmentation;
and 2) the relevance labels only come from the source corpus, leaving the augmentation training on other MoMA corpus lack of supervision.
Thus we propose to distill informative signals from the end task to guide the training process of our augmentation component.

Inspired by FiD~\citep{izacard2020distilling,izacard2022few}, we first consider distilling the encoder-decoder cross-attention scores aggregated from the dual encoder.
Ideally, the attention scores can be treated as a proxy of the relative importance of each augmentation document.
In FiD, it showed that for each augmenting document $d_i$, these scores can be aggregated across attention heads, layers and tokens to obtain a single score $w_i$ for $d_i$.
Given a non-augmented query $q$, denote the predicted ranking score for each augmenting document $d_i$ as $f(q, d_i)=\text{sim}(\mathbf{q}, \mathbf{d_i})$, FiD minimizes the KL-divergence between $w_i$ and $f(q, d_i)$.
The optimized $f(q, d_i)$ is then used to rank different augmentation documents and obtain the top $K$ documents as $A_K$ .

% The attention weight $w_i$ is then distilled to the grounder by minimizing its KL-divergence with the grounder predicted probability $f(q,g'_i)$:
% \begin{equation}
%     f(q,g'_i)=\frac{\exp{(s(q,g'_i)/t)}}{\sum^k_{i=1} \exp{(s(q,g'_i)/t)}},
% \end{equation}
% where $t$ is the softmax temperature to control how greedily the model learns from the distilled attention.
% The learning objective of the FiD grounder is minimizing KL$(w_i||f(q,g'_i))$.
We first try directly extending the original FiD setting from single augmentation corpus to MoMA.
In practice, we instantiate $f$ with the same T5 model architecture as the end task retriever $g$, but owning different parameters.
However, as shown in Section~\ref{sec:exp_distill}, it cannot guarantee a promising result on multiple corpus.
One possible reason could be the guidance provided by the soft attention is insufficient to distinguish informative documents from multiple memory components, especially when the relevance labels on most components are unavailable.
Moreover, the distillation loss only steers the model toward relevant augmentation documents, but it does not steer the model \textit{away} from irrelevant ones, which is a crucial lesson in building dense retrieval systems in previous works~\citep{xiong2020approximate,karpukhin2020dense}.

To alleviate the scarcity of negative feedback signals from the memory mixture, we sample hard negatives from the memory mixture and incorporate them in training.
We train the augmentation component using positive feedback signals from the end task and hard negatives sampled from the mixture in an iterative joint leaning setting.
During the beginning of the $t^{th}$ iteration, we first rerank all $K$ augmentation documents used in the last iteration according to their attention weights $w_{1:k}^{t-1}$.
We then transform the top $N$ ranked documents as pseudo positive augmentation documents, the binarized latent label $r_i$ is derived as:
\begin{align}
\label{equ:binarize}
    r^t_i=
    \begin{cases}
    1 , &w^{t-1}_i \in \text{Top N}_{i=1}^K w^{t-1}_i \\
    0  &w^{t-1}_i \in \text{Top N}_{i=1}^K w^{t-1}_i
    \end{cases}
\end{align}

The final positive training set $D_A^{t+}$ includes both relevance documents from the end task and $N$ pseudo positive grounding documents:
\begin{equation}
    D_A^{t+}=\{d_{r^t_i=1}\} \cup \{d_{g(q_{\text{aug}}, d)=1}\}
\end{equation}

The model then performs a round of fast approximate nearest neighbor (ANN) search according to the predicted ranking scores $f^{t-1}$ from the last iteration to construct hard negative set $D_A^{t-}$ from the entire memory mixture $\mathcal{M}$:
\begin{equation}
\label{equ:construct_aug}
    D_A^{t-} =
    \text{ANN}_{f^{t-1}} \setminus D_A^{t+}
\end{equation}
Through combining $D_A^{t+}$ and $D_A^{t-}$ as the complete training set $D_A^{t}$ for the augmentation component, we guarantee a comprehensive coverage of different components by including both positive and negative feedback signals from them. 

After training the augmentation component with $D_A^{t}$, we leverage its updated top prediction on $\mathcal{M}$ to construct the new augmentation set $A^t_K$.
The end task retriever take $A^t_K$ along with original query $q$ to update the augmented query:
\begin{align}
    \mathbf{q}^t_{\text{aug}}&=\text{Dec}([\text{Enc}(q), \text{Enc}(\text{[SEP]} d_1),...,\text{Enc}(\text{[SEP]} d_K)])), d_{1:K} \in A^t_K.
\end{align}

When training the end task retriever using relevant document set $D_C^{t+}$, \model{} first performs ANN searching to derive hard negative set $D_C^{t-}$ for augmented queries according to prediction scores $g^t$ on the source corpus $C_s$:
\begin{equation}
    D_C^{t-} =
    \text{ANN}_{g^{t-1}} \setminus D_C^{t+}, 
    g^t(q_{\text{aug}}, d)=\text{sim}(\mathbf{q}^t_{\text{aug}}, \mathbf{d}^t),
    \forall d^t \in  D_C^{t}
\end{equation}




It then tries to minimize the ranking loss $\mathcal{L}_r$ between all positive pairs $x_C^{t+} \in D_C^{t+}$ and hard negative pairs $x_C^{t-} \in D_C^{t-}$:
\begin{equation}
\label{equ:retriever_loss}
    \min_{\theta_g} \sum_{x_C^{t+} \in D_C^{t+}, x_C^{t-} \in D_C^{t-}} \mathcal{L}_r(g(x_C^{t+}),g(x_C^{t-})),
\end{equation}
where $\theta_g$ is the parameter set of the end task retriever.
After training the retriever for one iteration, we run inference on it to obtain the updated attention weight $w^t_i$ for each augmentation documents, and construct $D_A^{t+1}$ for a new round of augmentation training following Equation~\ref{equ:binarize}-\ref{equ:construct_aug}.
Similar with Equation~\ref{equ:retriever_loss}, the augmentation is trained by minimizing the ranking loss $\mathcal{L}_r$ on $D_A^{t+1}$:
\begin{equation}
\label{equ:grounder_loss}
    \min_{\theta_f} \sum_{x_A^{(t+1)+} \in D_A^{(t+1)+}, x_A^{(t+1)-} \in D_A^{(t+1)-}} \mathcal{L}_r(f(x_A^{(t+1)+}),f(x_A^{(t+1)-})).
\end{equation}
where $\theta_f$ is the parameter set of final retriever.

Following~\cite{xiong2020approximate}, we use dot product to measure similarity and set $\mathcal{L}_r$ as the negative log likelihood (NLL) loss.
During the iterative training process, we maintain two independent document index sets for $f$ and $g$, and only update them at the end of each training iteration.
Compared with naive retrieval augmented models, \model{} barely adds additional computational cost, while enjoying the merits of augmentation from multiple knowledge sources.

\textbf{Inference with Plug-in New Memories.}
As the final retrieval test bed, the target corpus is usually, if not always, the best-fit for in-domain adaptation.
To facilitate a flexible plug-in of different unseen targets, we swap out the source corpus $C_s$ in the memory mixture $\mathcal{M}$ during inference, and exchange it for target corpus $C_t$, i.e., $\mathcal{M}=\{C_t,C_1,C_2,...,C_M\}$.
The underlying assumption is that the model has absorbed the knowledge in the source corpus during training.
Thus we swap the target corpus to the same position, evoking the model to perform grounding on target in a similar manner.
Since the swapping process requires zero parameter modification, \model{} can be easily shipped to the end user for local usage even without accessing the local data.


















==> Arxiv/related.tex <==
\section{Related Work}

% \cx{Two main parts of related work, the retrieval augmented methods and the ZeroDR application methods}


% \cx{Retrieval augmented: start from the general motivation, go through the main methods that leverage retrieval augmentation. The actually implicit focus: 1) what retrieval corpus they use, indicating that they main using one given corpus that is often in domain  2) the method they use to learn the retrieval component, e.g., REALM and RETRO all use a fixed part, RAG has the distillation, and ALTLAS's different distillation methods. 3) what benefits they bring, especially on which tasks, showing that they often do it on application tasks where there is a retrieval component needed, like OpenQA and Fact verification to provide additional evidence}




% \cx{ZeroDR: 1) start with general dense retrieval how it has been 2) the challenge and importance of Zero-shot retrieval 3) previous techniques to improve generalization of retrieval}




% general RA models
There are two common ways to construct retrieval-augmentation for language models.
The first directly use all potential model outputs, i.e., \textit{tokens} in the vocabulary, as the corpus~\citep{khandelwal2019generalization}.
The retrieved nearest neighbor tokens augment the language models with 
an explicit set of high-quality candidate to predict the next token. Such token-based augmentation  has shown benefits on scenarios that emphasize on token prediction, such as machine translation~\citep{zhong2022training}.
The second one uses the standard \textit{document} corpus, for example, text sequences from the pretraining corpus. There the retrieved documents provide additional contexts in the input of language models~\citep{guu2020realm, borgeaud2022improving}.
This document-based augmentation aligns well with many real world applications, for example, on OpenQA~\citep{chen2017reading}, retrieval augmented generation~\citep{lewis2020retrieval}, and many knowledge extensive tasks~\citep{petroni2020kilt}. It is the main focus of this work.



% how the augmentation is formed: as it is, e.g., unsupervised BERT, then a dense retriever (ANCE-PRF)
The document-based retrieval augmentation can be viewed as a retrieval task which is to find useful contexts for the language model to perform its task. It is often done by dense retrieval, which maps texts by their dense embeddings with simple similarity metrics~\citep{lee2019latent, karpukhin2020dense, xiong2020approximate}.
\citet{guu2020realm} uses raw BERT representations to retrieve documents in the pretraining corpus as the augmentation component in REALM.
\citet{borgeaud2022improving} uses the same unsupervised representation but from a larger text corpus in RETRO.
A challenge of using raw BERT representations is that they not as well calibrated~\citep{lu2021less, gao2021simcse}. 
\citet{izacard2020leveraging} and \citet{lewis2020retrieval} used supervised DPR~\citep{karpukhin2020dense} to augmented their language model for QA and language generation.
\citet{yu2021improving} uses the supervised dense retriever to augment itself for better supervised retrieval, which is a form of pseudo relevance feedback in search~\citep{lavrenko2017relevance}.

% joint learning of the two
A dense retriever optimized for retrieval as the end goal may not be the optimal augmentation component for the language model.
 As direct labels on the latent augmentation layer is seldom available, recent research explored various ways to jointly train the augmentation component and the augmented model using feedback signals from the end task.
 \citet{zhao2021distantly} developed an EM method that treats the augmentation documents as latent variables and the end task labels as explicit observation to train the latent augmentation model.
 \citet{izacard2020distilling} uses the aggregated Transformer cross-attention scores between the output sequence and the augmenting documents as soft labels.
 \citet{izacard2022few} explored various ways to distill end task signals to the augmentation model.
 These jointly learning methods often perform an iterative training process with the augmentation component and the augmented language model trained one by one using the updated version of each other.

% mixture of experts, mixture of skills, etc.
Using model mixtures to improve the prediction effectiveness and robustness is a widely applied technique in classic machine learning, for example, in boosting~\citep{chen2016xgboost}.
Recent exploration in deep learning is more on the mixture-of-experts (MoE) front~\citep{Fedus2022switch}, which combines a set of dense subnetworks (experts) and uses a routing mechanism to sparsely active experts based on inputs. 
MoE provides a way to efficiently scale up the language model parameter sizes and obtains robust effectiveness, compared with dense models at similar inference speed~\citep{du2022glam, zuo2021taming}.






% other ways for efficiency LM?
% METRO
% optimization
% data scales
There are other research explorations for efficient scaling of language models.
One promising direction is to pretrain language models using text sequence corrupted by another model~\citep{clark2020electra}, forming a learning curriculum with more informative training signals~\citep{meng2021coco, bajaj2022metro}.
Another direction is to improve the optimization process of deep neural networks for more stable and efficient training~\citep{liu2020understanding, liang2022no}.
Finding the right combination of language model size, pretraining steps, and pretraining data size can also leads to more efficient scaling in empirical studies~\citep{hoffmann2022training}.




% ZeroDR application
Zero-shot dense retrieval (ZeroDR) has drawn much attention recently from academia and industry~\citep{thakur2021beir,cpt, gtr}.
It provides a promising way to democratize search from resource rich scenarios (mainly web search) to all other search scenarios through the generalization power of neural representation models~\citep{modir, wang2021gpl},
which is more feasible than heavily engineered feature-based systems.
% With search as an important real world application, 
With retrieval as an important real-word application, an improved ZeroDR system can lead to rich real word impact both commercial wise and society wise, for example, in medical search and academic search~\citep{kim2022applications}.
When retrieval is used as the first stage of other language systems, zero-shot is also often the case as direct training signals at the retrieval stage is hard to obtain. 























